In-Context Learning for Extreme Multi-Label Classification

Multi-label classification problems with thousands of classes are hard to solve with in-context learning alone, as language models (LMs) might lack prior knowledge about the precise classes or how to assign them, and it is generally infeasible to demonstrate every class in a prompt. We propose a general program, $\texttt{Infer--Retrieve--Rank}$, that defines multi-step interactions between LMs and retrievers to efficiently tackle such problems. We implement this program using the $\texttt{DSPy}$ programming model, which specifies in-context systems in a declarative manner, and use $\texttt{DSPy}$ optimizers to tune it towards specific datasets by bootstrapping only tens of few-shot examples. Our primary extreme classification program, optimized separately for each task, attains state-of-the-art results across three benchmarks (HOUSE, TECH, TECHWOLF). We apply the same program to a benchmark with vastly different characteristics and attain competitive performance as well (BioDEX). Unlike prior work, our proposed solution requires no finetuning, is easily applicable to new tasks, alleviates prompt engineering, and requires only tens of labeled examples. Our code is public at https://github.com/KarelDO/xmc.dspy.

==> ablation_table.tex <==
\begin{table*}[tp]
\centering
\begin{tabular}{@{}lllllllll@{}}
\toprule
                    & \multicolumn{2}{l}{BioDEX} & \multicolumn{2}{l}{HOUSE} & \multicolumn{2}{l}{TECH} & \multicolumn{2}{l}{TECHWOLF} \\ \cmidrule(l){2-9} 
                    & R@10        & RP@10        & R@10        & RP@10       & R@10       & RP@10       & R@10         & RP@10         \\ \midrule
Ours                &             &              &             &             &            &             &              &               \\
Ours -- compilation &             &              &             &             &            &             &              &               \\
Ours -- no prior    &             &              &             &             &            &             &              &               \\ \bottomrule
\end{tabular}
\caption{Ablations}
\label{table:ablation}
\end{table*}

==> data_table.tex <==
\begin{table*}[tp]
\centering
\begin{tabular}{@{}l|lll|l|ll}
\toprule
\multirow{2}{*}{dataset} & \multirow{2}{*}{train} & \multirow{2}{*}{dev} & \multirow{2}{*}{test} & \multirow{2}{*}{ontology items} & \multicolumn{2}{l}{labels per input}  \\
                         &                        &                      &                       &                                 & 50th              & 95th                      \\ \midrule
BioDEX                   & 100                       & 100                     & 500                       & 24,313                                 & 3                   & 14                                 \\ \midrule
HOUSE                    & 10                         & 51                      & 262                       & 13,896                                 & 1                   & 4                                  \\
TECH                     & 10                       & 65                      & 338                       & 13,896                                 & 1                   & 3                             \\
TECHWOLF                 & 20                        & 116                     & 326                      & 13,896                                 & 1                   & 4                                \\ \bottomrule
\end{tabular}
\caption{Data. \textcolor{blue}{TODO: put this into text, remove table}}
\label{table:data}
\end{table*}

==> results_table.tex <==
\begin{tabular}{lrrrrrrrr}
\toprule
model name & fulltext & 1 & 2 & 5 & 10 & 20 & 30 & 40 \\
\midrule
exact ngram match & False & 5.41 & 8.54 & 11.73 & 12.21 & 12.23 & 12.23 & 12.23 \\
exact ngram match & True & 4.43 & 7.63 & 15.47 & 24.91 & 31.50 & 32.70 & 32.98 \\
exact ngram match with prior & False & 5.54 & 9.13 & 15.94 & 22.98 & 28.96 & 32.45 & 34.77 \\
exact ngram match with prior & True & 4.43 & 7.63 & 15.49 & 25.00 & 33.68 & 40.06 & 44.95 \\
flan t5 large naive sort & False & 5.11 & 8.86 & 17.43 & 26.93 & 34.06 & 36.60 & 37.45 \\
flan t5 large voting sort & False & 7.13 & 14.31 & 23.84 & 31.05 & 35.78 & 37.19 & 37.55 \\
flan t5 large voting sort with prior & False & 7.13 & 14.37 & 24.57 & 33.35 & 41.70 & 46.16 & 49.03 \\
gold & False & 41.96 & 62.88 & 86.95 & 96.49 & 99.55 & 99.94 & 99.99 \\
iaa 1 vs 1 & False & 28.22 & 41.28 & 52.80 & 55.57 & 56.32 & 56.41 & 56.41 \\
iaa 1 vs all & False & 28.98 & 42.66 & 55.15 & 58.05 & 58.83 & 58.90 & 58.90 \\
iaa 1 vs rest & False & 24.40 & 35.71 & 45.84 & 48.28 & 48.89 & 49.00 & 49.00 \\
prior & False & 3.99 & 7.12 & 10.53 & 14.51 & 19.05 & 22.87 & 24.99 \\
\bottomrule
\end{tabular}


==> results_table2.tex <==
\begin{table*}[tp]
\begin{tabular}{@{}lllllllllllllllll@{}}
\toprule
                    & \multicolumn{4}{l}{BioDEX} & \multicolumn{4}{l}{TECH}  & \multicolumn{4}{l}{HOUSE} & \multicolumn{4}{l}{TECHWOLF} \\
                    & R@5  & R@10 & RP@5 & RP@10 & R@5 & R@10 & RP@5 & RP@10 & R@5 & R@10 & RP@5 & RP@10 & R@5  & R@10  & RP@5  & RP@10 \\ \midrule
\texttt{prior}               &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\
\texttt{ngram}               &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\
\texttt{retrieve}            &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\
\texttt{retrieve-fine tuned} &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\
\texttt{Llama-2-chat-naive}  &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\
\texttt{Llama-2-chat-expert} &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\
\texttt{Ours}                &      &      &      &       &     &      &      &       &     &      &      &       &      &       &       &       \\ \bottomrule
\end{tabular}
\caption{Results}
\label{table:results}
\end{table*}

==> results_table3.tex <==
\begin{table*}[tp]
\scriptsize
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr@{}}
\toprule
                    & \multicolumn{2}{l}{BioDEX} & \multicolumn{2}{l}{HOUSE} & \multicolumn{2}{l}{TECH} & \multicolumn{2}{l}{TECHWOLF} \\ \cmidrule(l){2-9} 
                    & RP@5        & RP@10        & RP@5        & RP@10       & RP@5       & RP@10       & RP@5         & RP@10         \\ \midrule
prior               & 20.42            & 21.51             & 2.90             & 2.97             & 1.63           & 1.63            &              & 2.57               \\
ngram               & 9.60            & 15.16             & 5.89             & 5.82             & 4.09            & 4.09             &              & 3.43              \\
retrieve            & 10.36             & 12.12             & 26.07            & 36.76            & 39.60            & 49.79             &              & 42.13              \\
retrieve (BioLORD)            & 10.99             & 11.71             & /            & /            & /            & /         & /             & /             \\
retrieve-fine tuned &             &              &             &             &            &             &              &               \\
Llama-2-chat-naive  &             &              &             &             &            &             &              &               \\
Llama-2-chat-expert &             &              &             &             &            &             &              &               \\ \midrule
Ours (uncompiled; K4P10000)               & 21.96            & 23.98             & 20.23             & 30.69             & 21.76            & 33.42            & 22.15              & 29.69              \\ \midrule
Ours (compiled; K4P10000)     & 23.19              & 27.20             &  42.80             & 53.79            & 49.06            & 60.25            & 47.72              & 53.60               \\ \midrule
Ours (comp + BioLORD; K4P10000)     & 24.55             & 29.37             & /             & /            & /            & /            & /              & /               \\ \midrule
Ours (uncompiled; swept per metric)               &           (2;8192) 30.40   & (2;8192) 27.45             & (2;256) 25.85               & (4;32) 28.71              & (4;2048) 35.9             & (4;256) 34.87            &     (2;4) 30.40           & (4;64) 30.08               \\ \midrule
Ours (swept per metric; then compile)               & 25.74            & 31.48             & 42.56             & 53.23               & 52.54            & 60.04             & 44.03              & 57.11               \\ \midrule
GPT4 re-ranking (best per metric) \\ \citep{clavie2023large}    &  /           & /             & 56.67            & 61.02             & 61.50           & 68.94            & /             & /              \\ \midrule
GPT-aug \citep{decorte2023extreme} & / & / & 45.74 & / & 54.62 & / & 54.57 & / \\ \bottomrule
\end{tabular}
\caption{Results}
\label{table:results}
\end{table*}

==> results_table4.tex <==
\begin{table*}[tp]
\scriptsize
\centering
\begin{tabular}{@{}l|rr|rr|rr|rr@{}}
\toprule
                    & \multicolumn{2}{l}{BioDEX} & \multicolumn{2}{l}{HOUSE} & \multicolumn{2}{l}{TECH} & \multicolumn{2}{l}{TECHWOLF} \\ \cmidrule(l){2-9} 
                    & RP@5        & RP@10        & RP@5        & RP@10       & RP@5       & RP@10       & RP@5         & RP@10         \\ \midrule
prior               & 20.42            & 21.51             & 2.90             & 2.97             & 1.63           & 1.63            &              & 2.57               \\
ngram               & 9.60            & 15.16             & 5.89             & 5.82             & 4.09            & 4.09             &              & 3.43              \\
retrieve            & 10.36             & 12.12             & 26.07            & 36.76            & 39.60            & 49.79             &              & 42.13              \\
retrieve (BioLORD)            & 10.99             & 11.71             & /            & /            & /            & /         & /             & /             \\
retrieve-fine tuned &             &              &             &             &            &             &              &               \\
Llama-2-chat-naive  &             &              &             &             &            &             &              &               \\
Llama-2-chat-expert &             &              &             &             &            &             &              &               \\ \midrule
Ours (uncompiled; K4P10000)               & 21.96            & 23.98             & 20.23             & 30.69             & 21.76            & 33.42            & 22.15              & 29.69              \\ \midrule
Ours (compiled; K4P10000)     & 23.19              & 27.20             &  42.80             & 53.79            & 49.06            & 60.25            & 47.72              & 53.60               \\ \midrule
Ours (comp + BioLORD; K4P10000)     & 24.55             & 29.37             & /             & /            & /            & /            & /              & /               \\ \midrule
Ours (uncompiled; swept per metric)               &           (2;8192) 30.40   & (2;8192) 27.45             & (2;256) 25.85               & (4;32) 28.71              & (4;2048) 35.9             & (4;256) 34.87            &     (2;4) 30.40           & (4;64) 30.08               \\ \midrule
Ours (swept per metric; then compile)               & 25.74            & 31.48             & 42.56             & 53.23               & 52.54            & 60.04             & 44.03              & 57.11               \\ \midrule
GPT4 re-ranking (best per metric) \\ \citep{clavie2023large}    &  /           & /             & 56.67            & 61.02             & 61.50           & 68.94            & /             & /              \\ \midrule
GPT-aug \citep{decorte2023extreme} & / & / & 45.74 & / & 54.62 & / & 54.57 & / \\ \bottomrule
\end{tabular}
\caption{Results}
\label{table:results}
\end{table*}

==> results_table5.tex <==
\begin{table*}[tp]
\small
\begin{tabular}{@{}l|llll|llll|llll|llll|@{}}
\cmidrule(l){2-17}
                                                                                                                                                            & \multicolumn{4}{l|}{BioDEX}                                                                                                                                                                                                                                                               & \multicolumn{4}{l|}{HOUSE}                                                                             & \multicolumn{4}{l|}{TECH}                                                                              & \multicolumn{4}{l|}{TECHWOLF}                                                                          \\ \midrule
\multicolumn{1}{|l|}{}                                                                                                                                      & \multicolumn{2}{l|}{RP@5}                                                                                                                              & \multicolumn{2}{l|}{RP@10}                                                                                                       & \multicolumn{2}{l|}{RP@5}                                    & \multicolumn{2}{l|}{RP@10}              & \multicolumn{2}{l|}{RP@5}                                    & \multicolumn{2}{l|}{RP@10}              & \multicolumn{2}{l|}{RP@5}                                    & \multicolumn{2}{l|}{RP@10}              \\ \midrule
\multicolumn{1}{|l|}{}                                                                                                                                      & \multicolumn{1}{l|}{validation}                                           & \multicolumn{1}{l|}{test}                                                  & \multicolumn{1}{l|}{validation}                                          & test                                                  & \multicolumn{1}{l|}{validation} & \multicolumn{1}{l|}{test}  & \multicolumn{1}{l|}{validation} & test  & \multicolumn{1}{l|}{validation} & \multicolumn{1}{l|}{test}  & \multicolumn{1}{l|}{validation} & test  & \multicolumn{1}{l|}{validation} & \multicolumn{1}{l|}{test}  & \multicolumn{1}{l|}{validation} & test  \\ \midrule
\multicolumn{1}{|l|}{\textbf{prior}}                                                                                                                        & \multicolumn{1}{l|}{9.38}                                                 & \multicolumn{1}{l|}{20.42}                                        & \multicolumn{1}{l|}{10.61}                                               & 21.51                                        & \multicolumn{1}{l|}{2.19}       & \multicolumn{1}{l|}{2.9}   & \multicolumn{1}{l|}{1.99}       & 2.97  & \multicolumn{1}{l|}{0.31}       & \multicolumn{1}{l|}{1.63}  & \multicolumn{1}{l|}{0.31}       & 1.63  & \multicolumn{1}{l|}{1.14}       & \multicolumn{1}{l|}{0.0}   & \multicolumn{1}{l|}{1.05}       & 2.57  \\
\multicolumn{1}{|l|}{exact match}                                                                                                                           & \multicolumn{1}{l|}{9.38}                                                 & \multicolumn{1}{l|}{9.6}                                                   & \multicolumn{1}{l|}{15.58}                                               & 15.16                                                 & \multicolumn{1}{l|}{10.13}      & \multicolumn{1}{l|}{5.89}  & \multicolumn{1}{l|}{10.13}      & 5.89  & \multicolumn{1}{l|}{8.21}       & \multicolumn{1}{l|}{4.09}  & \multicolumn{1}{l|}{8.21}       & 4.09  & \multicolumn{1}{l|}{9.05}       & \multicolumn{1}{l|}{3.43}  & \multicolumn{1}{l|}{9.05}       & 3.43  \\
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}dense retrieval (mpnet)\\ (bioLord)\end{tabular}}                                                           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}8.47\\ 11.62\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}10.36\\ 10.99\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}9.21\\ 11.0\end{tabular}} & \begin{tabular}[c]{@{}l@{}}12.12\\ 11.71\end{tabular} & \multicolumn{1}{l|}{40.98}      & \multicolumn{1}{l|}{26.17} & \multicolumn{1}{l|}{50.07}      & 36.76 & \multicolumn{1}{l|}{49.1}       & \multicolumn{1}{l|}{39.6}  & \multicolumn{1}{l|}{65.18}      & 49.79 & \multicolumn{1}{l|}{45.53}      & \multicolumn{1}{l|}{33.48} & \multicolumn{1}{l|}{58.53}      & 42.13 \\ \midrule
\multicolumn{1}{|l|}{ours (uncompiled)}                                                                                                                     & \multicolumn{1}{l|}{25.98}                                                & \multicolumn{1}{l|}{21.96}                                                 & \multicolumn{1}{l|}{28.12}                                               & 23.98                                                 & \multicolumn{1}{l|}{23.07}      & \multicolumn{1}{l|}{20.23} & \multicolumn{1}{l|}{31.63}      & 30.69 & \multicolumn{1}{l|}{33.46}      & \multicolumn{1}{l|}{21.76} & \multicolumn{1}{l|}{42.95}      & 33.42 & \multicolumn{1}{r|}{28.89}      & \multicolumn{1}{l|}{22.15} & \multicolumn{1}{l|}{37.97}      & 29.69 \\
\multicolumn{1}{|l|}{ours (best validation)}                                                                                                                & \multicolumn{1}{l|}{32.78}                                                & \multicolumn{1}{l|}{27.94}                                                 & \multicolumn{1}{l|}{37.20}                                               & 31.48                                                 & \multicolumn{1}{l|}{48.89}      & \multicolumn{1}{l|}{42.80} & \multicolumn{1}{l|}{54.44}      & 53.79 & \multicolumn{1}{l|}{73.77}      & \multicolumn{1}{l|}{52.54} & \multicolumn{1}{l|}{81.00}      & 60.04 & \multicolumn{1}{l|}{62.36}      & \multicolumn{1}{l|}{48.82} & \multicolumn{1}{l|}{70.40}      & 53.60 \\
\multicolumn{1}{|l|}{ours (sweep and compile)}                                                                                                              & \multicolumn{1}{l|}{32.78}                                                & \multicolumn{1}{l|}{27.94}                                                 & \multicolumn{1}{l|}{37.20}                                               & 31.48                                                 & \multicolumn{1}{l|}{43.37}      & \multicolumn{1}{l|}{42.56} & \multicolumn{1}{l|}{52.65}      & 52.20 & \multicolumn{1}{l|}{73.77}      & \multicolumn{1}{l|}{52.54} & \multicolumn{1}{l|}{81.0}       & 60.04 & \multicolumn{1}{l|}{57.18}      & \multicolumn{1}{l|}{44.03} & \multicolumn{1}{l|}{68.88}      & 57.11 \\ \midrule
\multicolumn{1}{|l|}{Decorte et al. 2023 best (gpt data + retrieve)}                                                                                        & \multicolumn{1}{l|}{/}                                                    & \multicolumn{1}{l|}{/}                                                     & \multicolumn{1}{l|}{/}                                                   &                                                       & \multicolumn{1}{l|}{/}          & \multicolumn{1}{l|}{45.74} & \multicolumn{1}{l|}{/}          & /     & \multicolumn{1}{l|}{/}          & \multicolumn{1}{l|}{54.62} & \multicolumn{1}{l|}{/}          & /     & \multicolumn{1}{l|}{/}          & \multicolumn{1}{l|}{54.57} & \multicolumn{1}{l|}{/}          & /     \\
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Clavi et al. 2023 (gpt data + class/retr + rerank) *\\ * selecting best per metric on test...\end{tabular}} & \multicolumn{1}{l|}{/}                                                    & \multicolumn{1}{l|}{/}                                                     & \multicolumn{1}{l|}{/}                                                   & /                                                     & \multicolumn{1}{l|}{/}          & \multicolumn{1}{l|}{56.67} & \multicolumn{1}{l|}{/}          & 61.02 & \multicolumn{1}{l|}{/}          & \multicolumn{1}{l|}{61.50} & \multicolumn{1}{l|}{/}          & 68.94 & \multicolumn{1}{l|}{/}          & \multicolumn{1}{l|}{/}     & \multicolumn{1}{l|}{/}          & /     \\ \bottomrule
\end{tabular}
\end{table*}
